Understanding and Benchmarking the Impact of GDPR on Database Systems

The General Data Protection Regulation (GDPR) provides new rights and protections to European people concerning their personal data. We analyze GDPR from a systems perspective, translating its legal articles into a set of capabilities and characteristics that compliant systems must support. Our analysis reveals the phenomenon of metadata explosion, wherein large quantities of metadata needs to be stored along with the personal data to satisfy the GDPR requirements. Our analysis also helps us identify new workloads that must be supported under GDPR. We design and implement an open-source benchmark called GDPRbench that consists of workloads and metrics needed to understand and assess personal-data processing database systems. To gauge the readiness of modern database systems for GDPR, we follow best practices and developer recommendations to modify Redis, PostgreSQL, and a commercial database system to be GDPR compliant. Our experiments demonstrate that the resulting GDPR compliant systems achieve poor performance on GPDR workloads, and that performance scales poorly as the volume of personal data increases. We discuss the real-world implications of these findings, and identify research challenges towards making GDPR compliance efficient in production environments. We release all of our software artifacts and datasets at http://www.gdprbench.org

==> revision.tex <==
\twocolumn[\Large \textbf{Response to Review for Paper 420 ``\textit{Understanding and Benchmarking the Impact of GDPR on Database Systems.''}}\newline]
\thispagestyle{empty}

We thank the individual reviewers and the meta-reviewer for providing insightful and actionable feedback. In this document, we present a summary of our new changes as well as our responses to all the suggested revision items. All of our modifications are colored in {\color{blue}blue}. We have put in our best faith effort in addressing all the concerns and incorporating the suggestions from the reviewers. We believe the paper has been significantly strengthened as a result.\newline

\noindent {\large{\bf Summary of Major Changes}\newline}
\label{sec-summary}

\vheading{1. Improved benchmark description.}
We include an in-depth discussion on the benchmark's implementation, data representation, and configuration (Reviewer-1 W2/D4). We fixed the inconsistency observed in the github repository (Reviewer-2).

\vheading{2. Improved evaluations.}
We evaluate Oracle DB, an enterprise-grade database system on GDPRbench, and report on our experiences with Microsoft SQL Server and Siodb (Meta-reviewer R2, Reviewer-1 W1/D2). We expand our scale experiments to 10GB (Reviewer-2 W2).

\vheading{3. Better calibration of the work.}
We distinguish this paper from our prior workshop report (Reviewer-2 W1). We reflect on our strict interpretation of GDPR (Reviewer-4 D2/D3, Reviewer-1 D5). We recalibrate the section on real-world implications (Reviewer-1 D3, Reviewer-2 W3). We elaborate on our choice of database systems (Reviewer-1 D1). We clarify our contributions in terms of what is newly designed/implemented vs. reused (Reviewer-1 W3). 

\noindent {\newline \large{\bf Reviewer-1}\newline}
\label{sec-r1}

\viheading{\textbf{W1.} The paper evaluates the efficiency of own implementation, instead of evaluating versus the state of the art.}

\viheading{\textbf{D3.} The paper re-implements common security features from scratch on Redis and PostgreSQL and evaluates them.}

\response{Our goal is to benchmark the state-of-the-art database systems against the requirements of GDPR. So, as for as possible, we have used the existing features, and resorted to third-party libraries or code changes only when no native support existed for the required features. We do realize that it may be possible to further improve the performance by undertaking GDPR-specific optimizations or by redesigning security mechanisms; it is not the focus of this work. We have clarified this in sec-1 limitations and sec-5 paragraph-1. 

Additionally, we strengthen our evaluation by integrating enter-prise-grade Oracle DB in sec-6. We also undertook evaluation of Microsoft SQL server and Siodb (results not included in the paper). While Microsoft SQL server has GDPR features that are comparable to that of Oracle, we were unable to get it operating at a similar level of baseline performance as Oracle DB, likely due to some configuration issues that were beyond us. We spent about two weeks debugging this, including posting on forums, but had no luck. Since we did not have access to professional SQL Server DBAs and since we believe Oracle DB suffices as a representative of enterprise-grade commercial RDBMS for empirical purposes (as suggested in the meta-review), we include additional results only for Oracle DB. Nevertheless, we offer a qualitative description of SQL Server's functionalities and discuss why it would perform similarly as Oracle DB under GDPR compliance in sec-5. Finally, Siodb is still under active development and we were told by its lead developer that its security features would not be ready before summer 2020.}

\viheading{\textbf{W2.} The benchmark is centered around key/value operations.} 

\response {The benchmark queries (listed in sec-3.3 and table-2a) are based on Create-Read-Update-Delete (CRUD) functionalities. This should map equally well to SQL and non-SQL architectures. In fact, we had to work harder to map GDPR queries to key-value operations than SQL.}

\viheading{\textbf{W2.} It doesn't investigate the impact of physical design decisions.} 

\response {Though the data representation chosen by the benchmark (in sec-4.2.1) has a resemblance to key-value format, the client stubs always reformat it match the native data layout of the selected database. We further clarify this in sec-4.2.1. We describe our current choices for data layouts for each of the three systems in sec-5. We also clarify that while the physical data layout and schema configurations impact the benchmark performance, these are external to the benchmark itself.}

\viheading{\textbf{W3.} I could not discern the systems contribution.}

\response{We thank the reviewer for the catch. We clarify that we do not claim novel systems contributions. We have removed lines that may suggest otherwise. As an E\&A paper, our contributions are three-fold, as listed at the end of sec-1: (i) analysis of the implications of GDPR for DB systems, (ii) design and implementation of the GDPRbench benchmark, and (iii) using GDPRbench to empirically evaluate the performance impact on three different representative DB systems (Redis, PostgreSQL, and Oracle).}

\viheading{\textbf{D1.} It would be great if the presentation conveyed how Redis and PostgreSQL represent specific instances of two broad categories.}

\response{We expanded sec-5 paragraph-1 to emphasize on the representativeness of the selected systems.} 

\viheading{\textbf{D2.} Address whether the current mechanisms suffice for GDPR compliance, or delve into technical details on how the current mechanisms need to change to achieve GDPR compliance.}

\response{Our evaluations indicate that even with native support for GDPR features, the current generation database systems suffer from performance degradation. We layout our reasoning for this in sec-7 and then propose on research directions that could help achieve compliance efficiently.}

\viheading{\textbf{D4.} The actual benchmark is described in vaguely in a single paragraph in Section 4.3.}

\response{We explain how the data is represented and stored in each of the systems in Sec-4.3 paragraph-3. We have set up secondary indices for both PostgreSQL and Oracle (updated sec-5 to reflect this). Redis' lack of support for high-level GDPR queries is managed by implementing wrapper routines in its database stub (sec-4.3 paragraph-3). We address the scalability and configurability of GDPRbench in sec-4.3 paragraph-4. We have also added a table in sec-5 to succinctly represent the natively supported features in each of our database systems.}

\viheading{\textbf{D5.} Curious whether the GDPR time-to-live clause is more demanding than the current state of the art.}

\response{GDPR has refrained from setting numerical thresholds for TTL (or from making any specific technological recommendations). We discuss how this turns compliance into a spectrum and its resulting implications in sec-1 paragraph-4, and in sec-7 paragraph-5.}

\viheading{\textbf{D6-D8.} Presentation comments.}

\response{Fixed inconsistencies in sec-10, and improved the narrative in sec-1 paragraph-1.}

\noindent {\newline \large{\bf Reviewer-2}\newline}
\label{sec-r1}
\thispagestyle{empty}

\viheading{\textbf{W1.} The first 5 pages of the paper are already published at HotStorage2019.}

\response{We clarify that HotStorage is a non-archival venue without proceedings; thus, we are compliant with VLDB's policy. HotStorage is just a forum for sharing preliminary work, limited to 5 pages. In fact, we conceived the idea for GDPR benchmark following our interactions with researchers and industry participants at HotStorage. Nevertheless, we have trimmed the background section to reduce overlap with the workshop paper. 

Here are the key additions in this paper vis-a-vis HotStorage version: (i) \textbf{Expanded analysis:} we identify the phenomenon of metadata explosion, and the list of GDPR queries (sec-3.1, 3.3); we provide a database perspective on GDPR (sec-2.2, fig-1); we reflect on the implementation challenges in the wild (sec-2.3), (ii) the \textbf{GDPR benchmark} is completely new (sec-4), and (iii) \textbf{Expanded evaluation:} HotStorage considered only Redis, and evaluated against just YCSB. In contrast, this paper expands the scope to PostgreSQL and Oracle (sec-5), and evaluates them in greater depth using GDPRbench (sec-6.2, 6.3). Finally, we discuss the real-world implications of our findings (sec-7).}

\viheading{\textbf{W2.} The depth of evaluation is rather shallow.}

\response{We strengthen our evaluation by integrating an enterprise-grade DB (Oracle). We tried to test a GDPR-oriented database (Siodb) but were told by its lead developer, Nicolas Penot, that its security features are still under active development. So it is not possible to show results with it yet. Next, in terms of scale experiments, we expand the dataset size for traditional workloads (YCSB) to 10GB. Since the database systems do not show good scalability for GDPR workloads, and instead become debilitatingly slow at GB scale, we limit the our experiment to 500MB. We acknowledge that this does not represent the scale of large telcos and social media companies, but would like to emphasize that GDPRbench in itself has no restriction on scaling either the dataset size or workload count. The updated sec-5 addresses these points.

Lastly, we do not attach any semantic meaning to personal data within the database. We treat each individual data item as a separate entity with its own GDPR metadata. However, the reviewer's comment on GPS traces raises interesting possibilities for data controllers to group related personal data items so that they share the same metadata, which in turn alters the performance tradeoff. We elucidate on this in sec-3.1 but due to space constraints, defer it to future work to study an expansion of our benchmark and experimental comparison that more holistically considers the semantics of personal data.} 

\viheading{\textbf{W3.} The technical consequences of GDPR are described with one particular way of dealing with them in mind.}

\response{As we clarify in sec-1 paragraph-4, we make a strict interpretation of GDPR. The reviewer's observation that GDPR could be interpretted in different (possibly less impacting) ways is valid. However, we believe that it is valuable to understand the worst-case performance impact resulting from a strict interpretation of GDPR articles.}

\viheading{\textbf{W3.} It appears that this work tests one particular strategy of GDPR compliance, and probably not the best one.}

\response{Our goal is to benchmark the state-of-the-art database systems against the requirements of GDPR. Thus, our compliance efforts (in sec-5) reuse the existing mechanisms and follow the official best practices. The reviewer's observation that performance impact could be lessened by targeted optimizations, redesign of security features etc., is valid. While we highlight these directions in sec-7 last paragraph, we do not implement or evaluate them because such new systems optimizations are not part of our goals in this particular E\&A paper. We leave it to a future research paper to study new systems optimizations and note that GDPRbench can help assess the impact of such optimizations in the future.}

\viheading{It was observed that in case of the SQL implementation (postrgresql), the get-log action is a no-op}

\response{Thanks for notifying us. We have confirmed that the results were based on the correct code, and will update github repository to the latest. We have also clarified the language in sec-5 to reflect that our GDPR-compliant PostgreSQL and Oracle DBs create their audit logs during the query time itself and simply return the requested portions of the log from a master log file. We do not support audit trail reconstruction in a manner indicated by the reviewer.}

\noindent {\newline \large{\bf Reviewer-4}\newline}
\label{sec-r1}

\viheading{\textbf{W1.} The paper proves what anyone would expect.}

\response{While our top-line results are not unexpected, we believe that a systematic evaluation of even predictable outcomes is helpful in advancing the field. In addition, our work makes several novel contributions (i) analyzing GDPR requirements from a database perspective, (ii) designing a benchmark that allows DB developers and admins in evaluating their systems, and (iii) highlighting the research and real-world challenges of operating GDPR-compliant databases.}

\viheading{\textbf{W2.} The paper explores only the straightforward solution of adding the metadata within the data records.}

\response{Kindly see our response for Reviewer-2 W3. As we describe in sec-4.3, GDPRbench does not mandate any particular physical data layout and leaves it up to the database to determine the best option. Since this is external to the benchmark, we have omitted a detailed investigation of the resulting tradeoffs.}

\viheading{\textbf{W3.} the work should be extended with the exploration of solutions that do logging more efficiently.}

\response{Unfortunately, none of the contemporary database systems in our evaluation supported efficient mechanisms for auditing or logging. Interestingly, though Oracle DB natively supported auditing, the results in sec-5 show that it is not efficient under GDPR settings. However, designing new mechanisms for efficient logging is beyond the scope of this work. We have expanded sec-7 to highlight some possible directions.}

\viheading{\textbf{D2.} Metadata can be stored separately and updated in a lazy manner, taking into account the application in hand. Also, metadata could be stored not per record but per person.}

\response{It may be possible to share GDPR metadata between a group of closely related records (say, GPS coordinates of a person). However, metadata cannot be the same across all data belonging to a person. For example, a person's SSN numbers will have different metadata characteristics than their search history. We present an updated discussion on this in sec-3.1. 

Yes, storing metadata separately from data or normalizing metadata across different records provide interesting tradeoff between storage overhead and access latency. These are exactly the kind of experiments we envision DBAs and DB designers to be performing using GDPRbench. This paper's key contribution is the benchmark itself and the empirical study that demonstrates the resultant interesting performance-compliance tradeoffs. New systems-level techniques to optimize the tradeoffs are beyond the scope of this E\&A paper, and we leave it to a future research paper to study such techniques.}

\viheading{Deleting the data/metadata with some laziness seems an acceptable solution.}

\response{Lazy deletion may be acceptable since GDPR does not specify how soon after a request, should the data be removed. Also, we do not yet have any legal precedences on what constitutes as a reasonable deletion timeline. However, we take a strict interpretation of GDPR articles, and include the time-taken-for-deletion in the overall completion time. We deliberate on this choice in sec-1 paragraph-4.}

\thispagestyle{empty}


